Accelerating 3D Deep Learning with PyTorch3D

Deep learning has significantly improved 2D image recognition. Extending into 3D may advance many new applications including autonomous vehicles, virtual and augmented reality, authoring 3D content, and even improving 2D recognition. However despite growing interest, 3D deep learning remains relatively underexplored. We believe that some of this disparity is due to the engineering challenges involved in 3D deep learning, such as efficiently processing heterogeneous data and reframing graphics operations to be differentiable. We address these challenges by introducing PyTorch3D, a library of modular, efficient, and differentiable operators for 3D deep learning. It includes a fast, modular differentiable renderer for meshes and point clouds, enabling analysis-by-synthesis approaches. Compared with other differentiable renderers, PyTorch3D is more modular and efficient, allowing users to more easily extend it while also gracefully scaling to large meshes and images. We compare the PyTorch3D operators and renderer with other implementations and demonstrate significant speed and memory improvements. We also use PyTorch3D to improve the state-of-the-art for unsupervised 3D mesh and point cloud prediction from 2D images on ShapeNet. PyTorch3D is open-source and we hope it will help accelerate research in 3D deep learning.

==> figures/silh_cloud_render/silh_cloud_render.tex <==
\begin{figure}
  \caption{Shape reconstruction via silhouette point cloud rendering on the ShapeNet test set. We show the input image, the predicted 3D point cloud and an additional random view.}
  \label{fig:silh_cloud_render}
  \centering
  \begin{minipage}{0.3\linewidth}\centering Input \end{minipage}
  \begin{minipage}{0.6\linewidth}\centering Point Align \end{minipage}
    % {left lower right upper}
  \includegraphics[width=0.3\linewidth]{figures/silh_cloud_render/inputs/03001627-d4326cd55ed8333f6a059e1fc701f06-10}
  \includegraphics[width=0.3\linewidth]{figures/silh_cloud_render/pointalign/03001627-d4326cd55ed8333f6a059e1fc701f06-10_blender000}
  \includegraphics[width=0.3\linewidth]{figures/silh_cloud_render/pointalign/03001627-d4326cd55ed8333f6a059e1fc701f06-10_rot_blender000} \\
  
  \includegraphics[width=0.3\linewidth]{figures/silh_cloud_render/inputs/04379243-ea60ea168f766580617092ec6e36103f-01}
  \includegraphics[width=0.3\linewidth]{figures/silh_cloud_render/pointalign/04379243-ea60ea168f766580617092ec6e36103f-01_blender000}
  \includegraphics[width=0.3\linewidth]{figures/silh_cloud_render/pointalign/04379243-ea60ea168f766580617092ec6e36103f-01_rot_blender000}
  \vspace{-4mm}
\end{figure}


==> figures/silh_mesh_render/silh_mesh_render.tex <==
\begin{figure}
  \centering
  \begin{minipage}{0.13\linewidth}\centering Input \end{minipage}
  \begin{minipage}{0.26\linewidth}\centering Sphere FC \end{minipage}
  \begin{minipage}{0.26\linewidth}\centering Sphere GCN \end{minipage}
  \begin{minipage}{0.26\linewidth}\centering Voxel GCN \end{minipage} \\*
  % {left lower right upper}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/inputs/02691156-d54ca25127a15d2b937ae00fead8910d-11}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/02691156-d54ca25127a15d2b937ae00fead8910d-11_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/02691156-d54ca25127a15d2b937ae00fead8910d-11_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/02691156-d54ca25127a15d2b937ae00fead8910d-11_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/02691156-d54ca25127a15d2b937ae00fead8910d-11_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/02691156-d54ca25127a15d2b937ae00fead8910d-11_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/02691156-d54ca25127a15d2b937ae00fead8910d-11_blender_rotated000} \\

  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/inputs/02828884-f1252c297d7ad9a47c51ec7d2716b33d-03}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/02828884-f1252c297d7ad9a47c51ec7d2716b33d-03_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/02828884-f1252c297d7ad9a47c51ec7d2716b33d-03_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/02828884-f1252c297d7ad9a47c51ec7d2716b33d-03_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/02828884-f1252c297d7ad9a47c51ec7d2716b33d-03_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/02828884-f1252c297d7ad9a47c51ec7d2716b33d-03_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/02828884-f1252c297d7ad9a47c51ec7d2716b33d-03_blender_rotated000} \\

  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/inputs/03001627-d0cf0982f16e5d583178d91f48c2217-07}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/03001627-d0cf0982f16e5d583178d91f48c2217-07_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/03001627-d0cf0982f16e5d583178d91f48c2217-07_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/03001627-d0cf0982f16e5d583178d91f48c2217-07_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/03001627-d0cf0982f16e5d583178d91f48c2217-07_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/03001627-d0cf0982f16e5d583178d91f48c2217-07_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/03001627-d0cf0982f16e5d583178d91f48c2217-07_blender_rotated000} \\

  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/inputs/03001627-ea762c2f1c6e966be464faca7dae7fdd-23}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/03001627-ea762c2f1c6e966be464faca7dae7fdd-23_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/03001627-ea762c2f1c6e966be464faca7dae7fdd-23_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/03001627-ea762c2f1c6e966be464faca7dae7fdd-23_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/03001627-ea762c2f1c6e966be464faca7dae7fdd-23_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/03001627-ea762c2f1c6e966be464faca7dae7fdd-23_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/03001627-ea762c2f1c6e966be464faca7dae7fdd-23_blender_rotated000} \\

  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/inputs/03001627-d4326cd55ed8333f6a059e1fc701f06-12}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/03001627-d4326cd55ed8333f6a059e1fc701f06-12_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/03001627-d4326cd55ed8333f6a059e1fc701f06-12_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/03001627-d4326cd55ed8333f6a059e1fc701f06-12_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/03001627-d4326cd55ed8333f6a059e1fc701f06-12_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/03001627-d4326cd55ed8333f6a059e1fc701f06-12_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/03001627-d4326cd55ed8333f6a059e1fc701f06-12_blender_rotated000} \\

  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/inputs/04379243-eca46f21f2893069c0a61ad1cf92b694-10}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/04379243-eca46f21f2893069c0a61ad1cf92b694-10_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/04379243-eca46f21f2893069c0a61ad1cf92b694-10_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/04379243-eca46f21f2893069c0a61ad1cf92b694-10_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/04379243-eca46f21f2893069c0a61ad1cf92b694-10_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/04379243-eca46f21f2893069c0a61ad1cf92b694-10_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/04379243-eca46f21f2893069c0a61ad1cf92b694-10_blender_rotated000} \\

  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/inputs/04379243-f7e7473775d8c3f3f51fa0238791f5dc-04}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/04379243-f7e7473775d8c3f3f51fa0238791f5dc-04_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spherefc/04379243-f7e7473775d8c3f3f51fa0238791f5dc-04_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/04379243-f7e7473775d8c3f3f51fa0238791f5dc-04_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/spheregcn/04379243-f7e7473775d8c3f3f51fa0238791f5dc-04_blender_rotated000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/04379243-f7e7473775d8c3f3f51fa0238791f5dc-04_blender000}
  \includegraphics[width=0.13\linewidth]{figures/silh_mesh_render/voxelgcn/04379243-f7e7473775d8c3f3f51fa0238791f5dc-04_blender_rotated000} \\
  
  \caption{Shape reconstruction predictions via silhouette mesh rendering on the ShapeNet test set. We show the input image (left). For each model, we show the object shape prediction made the model and an additional random view.}
  \label{fig:silh_mesh_render}
  \vspace{-4mm}
\end{figure}


==> figures/text_cloud_render/text_cloud_render.tex <==
% \begin{figure}
\begin{wrapfigure}{r}{6cm}
  \centering
  \small
  \begin{minipage}{0.32\linewidth}\centering  \small Input \end{minipage}
  \begin{minipage}{0.32\linewidth}\centering \small Alpha \end{minipage}
  \begin{minipage}{0.32\linewidth}\centering \small Norm \end{minipage}  \\*
  % {left lower right upper}
  \includegraphics[trim=0 31 0 31,clip,width=0.32\linewidth]{figures/text_cloud_render/inputs/02958343-f8e415203a26f77cd0d539ff39d45962-20}
  \includegraphics[trim=0 31 0 31,clip,width=0.32\linewidth]{figures/text_cloud_render/alpha/02958343-f8e415203a26f77cd0d539ff39d45962-20_rendered}   
  \includegraphics[trim=0 31 0 31,clip,width=0.32\linewidth]{figures/text_cloud_render/norm/02958343-f8e415203a26f77cd0d539ff39d45962-20_rendered}

  \caption{Point cloud and texture predictions via textured rendering on the ShapeNet test set.}
  \label{fig:text_cloud_render}
  \vspace{-4mm}
% \end{figure}
\end{wrapfigure}


==> figures/text_mesh_render/text_mesh_render.tex <==
\begin{figure}
  \centering
  \begin{minipage}{0.13\linewidth}\centering Input \end{minipage}
  \begin{minipage}{0.26\linewidth}\centering Flat \end{minipage}
  \begin{minipage}{0.26\linewidth}\centering Phong \end{minipage}
  \begin{minipage}{0.26\linewidth}\centering Gouraud \end{minipage} \\*
  % {left lower right upper}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/inputs/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/flat/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_blender000}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/flat/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_rendered_rgba}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/phong/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_blender000}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/phong/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_rendered_rgba}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/gouraud/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_blender000}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/gouraud/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_rendered_rgba} \\

  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/inputs/02958343-d832626f2bee7407290fad8e3fdaf4fe-21}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/flat/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/flat/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/phong/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/phong/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/gouraud/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=0.13\linewidth]{figures/text_mesh_render/gouraud/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba} \\

  \caption{Shape and texture reconstruction predictions via texture mesh rendering on the ShapeNet test set. We show the input image (left). For each shading function, we show the shape prediction and its textured rendering as predicted by the model.}
  \label{fig:text_mesh_render}
  \vspace{-4mm}
\end{figure}


==> figures/text_mesh_render/text_mesh_render_v2.tex <==
\begin{figure}
  \centering
  \begin{minipage}{1.5cm} \hspace{0.1cm} Model \end{minipage}
  \begin{minipage}{1.5cm}\centering Input \end{minipage}
  \begin{minipage}{3cm}\centering Flat \end{minipage}
  \begin{minipage}{3cm}\centering Phong \end{minipage}
  \begin{minipage}{3cm}\centering Gouraud \end{minipage} \\*
  % {left lower right upper}
  \FramedBox{1.5cm}{1.5cm}{Voxel GCN}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/inputs/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/flat/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/flat/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_rendered_rgba}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/phong/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/phong/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_rendered_rgba}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/gouraud/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/gouraud/voxelgcn/03001627-d6ac690c293a492d2d2a5d4c4022b4c6-08_rendered_rgba} \\

  \FramedBox{1.5cm}{1.5cm}{Voxel GCN}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/inputs/02958343-d832626f2bee7407290fad8e3fdaf4fe-21}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/flat/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/flat/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/phong/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/phong/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/gouraud/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/gouraud/voxelgcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba} \\

  \FramedBox{1.5cm}{1.5cm}{Sphere GCN}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/inputs/02958343-d832626f2bee7407290fad8e3fdaf4fe-21}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/flat/spheregcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/flat/spheregcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/phong/spheregcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/phong/spheregcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/gouraud/spheregcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_blender000}
  \includegraphics[width=1.5cm]{figures/text_mesh_render/gouraud/spheregcn/02958343-d832626f2bee7407290fad8e3fdaf4fe-21_rendered_rgba} \\

  \caption{Shape and texture predictions via textured mesh rendering on the ShapeNet test set. We show the input image (left). For each shading function, we show the shape prediction and its textured rendering as predicted by the model.}
  \label{fig:text_mesh_render}
  \vspace{-4mm}
\end{figure}

